Addressing Heterogeneity in Federated Load Forecasting with Personalization Layers

The advent of smart meters has enabled pervasive collection of energy consumption data for training short-term load forecasting models. In response to privacy concerns, federated learning (FL) has been proposed as a privacy-preserving approach for training, but the quality of trained models degrades as client data becomes heterogeneous. In this paper we propose the use of personalization layers for load forecasting in a general framework called PL-FL. We show that PL-FL outperforms FL and purely local training, while requiring lower communication bandwidth than FL. This is done through extensive simulations on three different datasets from the NREL ComStock repository.

==> img2/diagram.tex <==
%\documentclass[tikz,border=1mm]{standalone}
%\usepackage{tikz}
%\usepackage{amsmath,amssymb}
\usetikzlibrary{positioning, calc}%
\usetikzlibrary{arrows.meta}%
\usetikzlibrary{positioning,shapes,shadows,arrows}%
%
%\tikzstyle{abstract}=[rectangle, draw=black, rounded corners, fill=blue!30, drop shadow,
%text centered, anchor=north, text width=5cm]
%\tikzstyle{abstract2}=[rectangle, draw=black, rounded corners, fill=green!30, drop shadow,
%text centered, anchor=north, text width=5cm]
%\tikzstyle{myarrow}=[->, >=open triangle 90, thick]
%
\def\shift{5pt}%
\def\scaledShift{8pt}%
\def\pad{3pt}%
\def\clsep{5cm}%
%\begin{document}\textsl{\textsl{}}
		\begin{tikzpicture}
			\node (server) [abstract, rectangle split, rectangle split parts=3]
			{
				\textbf{{Server}}
				\nodepart{second}\textbf{Storage}\\
				Cent-FL-STLF: $\pmb{\theta}_k$\\
				PL-FL-STLF: $\pmb{\phi}_k$
				\nodepart{third}\textbf{Update}\\
				Cent-FL-STLF: Algorithm~\ref{alg:cent-fl}, lines \ref{line:CentServerStart}-\ref{line:CentServerEnd}\\
				PL-FL-STLF: Algorithm~\ref{alg:pers-fl}, lines \ref{line:PLServerStart}-\ref{line:PLServerEnd}
			};
			%\node (ClientNode) [text width=4cm, below=of server] {};
%			\node (client1) [abstract2, rectangle split, rectangle split parts=3, left=\clsep of ClientNode]
%			{
%				\textbf{Client 1}
%				\nodepart{second}\textbf{Storage}\\
%				Cent-FL-STLF: $\mcal{D}_1$\\
%				PL-FL-STLF: $\mcal{D}_1,\pmb{\psi}^1_{k}$
%				\nodepart{third}\textbf{Update}\\
%				Cent-FL-STLF: Algorithm~\ref{alg:cent-fl}, lines \ref{line:CentClientStart}-\ref{line:CentClientEnd}\\
%				PL-FL-STLF: Algorithm~\ref{alg:pers-fl}, lines \ref{line:CentServerStart}-\ref{line:CentServerEnd}
%			};
			\node (clientN) [abstract2, rectangle split, rectangle split parts=3, right=\clsep of server]
			{
				\textbf{Client $m$}
				\nodepart{second}\textbf{Storage}\\
				Cent-FL-STLF: $\mcal{D}_m$\\
				PL-FL-STLF: $\mcal{D}_m,\pmb{\psi}^m_{k}$
				\nodepart{third}\textbf{Update}\\
				Cent-FL-STLF: Algorithm~\ref{alg:cent-fl}, lines \ref{line:CentClientStart}-\ref{line:CentClientEnd}\\
				PL-FL-STLF: Algorithm~\ref{alg:pers-fl}, lines \ref{line:PLClientStart}-\ref{line:PLClientEnd}
			};
		%
%			\node (client2) [abstract2, rectangle split, rectangle split parts=3] at (ClientNode)
%			{
%				\textbf{Client 2}
%				\nodepart{second}\textbf{\texttt{Storage:}}
%				$\mathcal{D}_2$
%				\nodepart{third}\texttt{Update:} Algorithm X, $a$-$b$
%			};
		%
			\draw[myarrow] ([yshift=\shift] server.east) -- ([yshift=\shift] clientN.west) node [midway, above, sloped,align=center] (cmto) {Cent-FL-STLF: $\pmb{\theta}_k$\\PL-FL-STLF: $\pmb{\phi}_k$};
			\draw[myarrow] ([yshift=-\shift]clientN.west) -- ([yshift=-\shift]server.east) node [midway, below, sloped,align=center] (cmfrom) {$\tilde{\pmb{g}}^m_k$};
			%
			%\draw [brown] (current bounding box.south west) rectangle (current bounding box.north east);
			%
%			\draw[myarrow] ([xshift=-\scaledShift,yshift=-\pad] server.south) -- ([xshift=-\scaledShift,yshift=\pad] client2.north) node [midway, above, sloped,rotate=180] (c2to) {$\pmb{\theta}_k$};
%			\draw[myarrow] ([xshift=\scaledShift,yshift=\pad]client2.north) -- ([xshift=\scaledShift,yshift=-\pad]server.south) node [midway, below, sloped] (c2from) {$\tilde{\pmb{g}}^2_k$};
%			
%			\draw[myarrow] ([xshift=-\shift,yshift=\shift] server.south west) -- ([xshift=-\shift,yshift=\shift] client1.north east) node [midway, above, sloped] (c1to) {$\pmb{\theta}_k$};
%			\draw[myarrow] ([xshift=\shift,yshift=-\shift]client1.north east) -- ([xshift=\shift,yshift=-\shift]server.south west)  node [midway, below, sloped] (c1from) {$\tilde{\pmb{g}}^1_k$};
			
%			\draw[->] ([xshift=\shift,yshift=\shift] server.south) -- ([xshift=\shift,yshift=\shift]client2.north);
%			\draw[->] ([xshift=-\shift,yshift=-\shift] client2 ) -- ([xshift=-\shift,yshift=-\shift] server.south east);
		\end{tikzpicture}
%\end{document}
